An energy-based discontinuous Galerkin method for semilinear wave equations

We generalize the energy-based discontinuous Galerkin method proposed in [SIAM J. Num. Anal., 53(6):2705-2726, 2015.] to second-order semilinear wave equations. A stability and convergence analysis is presented along with numerical experiments demonstrating optimal convergence for certain choices of the interelement fluxes. Applications to the sine-Gordon equation include simulations of breathers, kink, and anti-kink solitons.

==> lurefs.tex <==
@article{appelo2015new,
  title={A new discontinuous {G}alerkin formulation for wave equations in second-order form},
  author={D. Appel\"o and T. Hagstrom},
  journal={SIAM J. Num. Anal.},
  volume={53},
  number={6},
  pages={2705--2726},
  year={2015}
}

@article{chou2014optimal,
  title={Optimal energy conserving local discontinuous {G}alerkin methods for second-order wave equation in heterogeneous media},
  author={C.-S. Chou, C.-W. Shu and Y. Xing},
  journal={J. Comput. Phys.},
  volume={272},
  pages={88--107},
  year={2014}
}

@book{ciarlet2002finite,
  title={The Finite Element Method for Elliptic Problems},
  author={P.~G. Ciarlet},
  volume={40},
  year={2002},
  series = {Classics in Applied Mathematics},
  publisher={SIAM}
}

@Article{zhang2019energy,
author = {L. Zhang, T. Hagstrom and D. Appel\"o},
title = {An energy-based discontinuous {G}alerkin method for the wave equation
with advection},
year = {2019},
journal = {SIAM J. Num. Anal.},
volume = {57},
pages = {2469-2492}
}

@Book{HesthavenWarburton08,
author = {J. Hesthaven and T. Warburton},
title = {Nodal Discontinuous Galerkin Methods},
publisher = {Springer-Verlag},
address = {New York},
series = {Texts in Applied Mathematics},
number = {54},
year = {2008}
}

@Article{el_dg_dath,
author={D. Appel\"o and T. Hagstrom},
title = {An energy-based discontinuous {G}alerkin discretization of the elastic wave
equation in second order form},
year={2018},
journal = {Computer Meth. Appl. Mech. Engrg.},
volume = {338},
pages = {362-391}
}

@Article{RiviereWheelerWave,
  title = {Discontinuous finite element methods for acoustic and elastic
wave problems},
  author = {B. Rivi\'ere and M. Wheeler},
  journal = {Contemp. Math.},
  year = {2003},
  volume = {329},
  pages = {271-282}
}

@Article{GSSwave,
  title = {Discontinuous {G}alerkin finite element method for the wave
equation},
  author = {M. Grote, A. Schneebeli and D. Sch\"otzau},
  journal = {SIAM J. Num. Anal.},
  volume = {44},
  year = {2006},
  pages = {2408-2431}
}

@Article{GodunovHDG,
   author = {T. Bui-Thanh},
   title = {From {G}odunov to a unified hybridized discontinuous {G}alerkin
   framework for partial differential equations},
   journal = {J. Comput. Phys.},
   volume = {295},
   pages = {114-146},
   year = {2015}
   }

@article{AURSAND2017478,
title = {Local discontinuous {G}alerkin schemes for a nonlinear variational wave equation
modelling liquid crystals},
journal = {J. Comput. Appl. Math.},
volume = {317},
pages = {478--499},
year = {2017},
author = {P. Aursand and U. Koley}
}

@Article{CiCP-23-747,
author = {N. Yi and H. Liu},
title = {An Energy Conserving Local Discontinuous {G}alerkin Method for a Nonlinear Variational
Wave Equation},
journal = {Commun. Comput. Phys.},
year = {2018},
volume = {23},
pages = {747--772}
}




